Differential Privacy Over Riemannian Manifolds

In this work we consider the problem of releasing a differentially private statistical summary that resides on a Riemannian manifold. We present an extension of the Laplace or K-norm mechanism that utilizes intrinsic distances and volumes on the manifold. We also consider in detail the specific case where the summary is the Fr\'echet mean of data residing on a manifold. We demonstrate that our mechanism is rate optimal and depends only on the dimension of the manifold, not on the dimension of any ambient space, while also showing how ignoring the manifold structure can decrease the utility of the sanitized summary. We illustrate our framework in two examples of particular interest in statistics: the space of symmetric positive definite matrices, which is used for covariance matrices, and the sphere, which can be used as a space for modeling discrete distributions.

==> DP Over Manifolds/latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> DP Over Manifolds/supplement_Arxiv.tex <==
% \documentclass{article}

% \RequirePackage[OT1]{fontenc}
% \RequirePackage{amsthm,amsmath}
% \RequirePackage[numbers]{natbib}

% \usepackage{xr-hyper}
% \RequirePackage{hyperref}

% \usepackage{bm,bbm}

% \usepackage{amssymb}
% \usepackage{amsthm}
% \usepackage{amsmath,color,comment}
% \usepackage{graphicx}

% \usepackage{mathrsfs}
% \DeclareMathAlphabet{\mathpzc}{OT1}{pzc}{m}{it} % load "Zapf Chancery" as a math alphabet


% \newcommand{\mone}{\mathbbm{1}}

% \newcommand{\mcA}{\mathcal{A}}
% \newcommand{\mbA}{\mathbb{A}}
% \newcommand{\mbB}{\mathbb{B}}
% \newcommand{\mcB}{\mathcal{B}}
% \newcommand{\mcC}{\mathcal{C}}
% \newcommand{\mcD}{\mathcal{D}}
% \newcommand{\mcc}{\mathpzc{c}}
% \newcommand{\mce}{\mathpzc{e}} %{\mathcalligra {e}}
% \newcommand{\mcE}{\mathcal{E}}
% \newcommand{\mcF}{\mathcal{F}}
% \newcommand{\bG}{{\bf G}}
% \newcommand{\mcG}{\mathcal{G}}
% \newcommand{\mcg}{\mathcal{g}}
% \newcommand{\mbH}{\mathbb{H}}
% \newcommand{\mcH}{\mathcal{H}}
% \newcommand{\mcI}{\mathcal{I}}
% \newcommand{\mcJ}{\mathcal{J}}
% \newcommand{\mcK}{\mathcal{K}}
% \newcommand{\mbK}{\mathbb{K}}
% \newcommand{\mcL}{\mathcal{L}}
% \newcommand{\mcM}{\mathcal{M}}
% \newcommand{\mcN}{\mathcal{N}}
% \newcommand{\mcP}{\mathcal{P}}
% \newcommand{\mbR}{\mathbb{R}}
% \newcommand{\mcS}{\mathcal{S}}
% \newcommand{\bt}{{\bf t}}
% \newcommand{\bU}{{\bf U}}
% \newcommand{\mbX}{\mathbb{X}}
% \newcommand{\mcX}{\mathcal{X}}
% \newcommand{\bX}{{\bf X}}

% \newcommand{\mbPk}{\mathbb{P}(k)}

% %\newcommand{\l}[1]{\left{#1}}
% %\newcommand{\r}[1]{\right{#1}}
% \newcommand{\ep}{\epsilon}
% \newcommand{\blue}{\textcolor{blue}}
% \newcommand{\red}{\textcolor{red}}
% \newcommand{\green}{\textcolor{green}}



% \newtheorem{theorem}{Theorem}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{claim}{Claim}
% \newtheorem{proposition}{Proposition}

% \theoremstyle{plain}
% \newtheorem{definition}{Definition}
% \newtheorem{example}{Example}

% \DeclareMathOperator{\cut}{cut}
% \DeclareMathOperator{\E}{E}
% \DeclareMathOperator{\Span}{span}
% \DeclareMathOperator{\Var}{Var}
% \DeclareMathOperator{\vech}{vech}
% \DeclareMathOperator*{\argmin}{argmin}

% \graphicspath{ {./images/} }

% \makeatletter
% \newcommand*{\addFileDependency}[1]{% argument=file name and extension
%   \typeout{(#1)}% latexmk will find this if $recorder=0 (however, in that case, it will ignore #1 if it is a .aux or .pdf file etc and it exists! if it doesn't exist, it will appear in the list of dependents regardless)
%   \@addtofilelist{#1}% if you want it to appear in \listfiles, not really necessary and latexmk doesn't use this
%   \IfFileExists{#1}{}{\typeout{No file #1.}}% latexmk will find this message if #1 doesn't exist (yet)
% }
% \makeatother

% \newcommand*{\myexternaldocument}[1]{%
%     \externaldocument{#1}%
%     \addFileDependency{#1.tex}%
%     \addFileDependency{#1.aux}%
% }

% \myexternaldocument{DP_Manifold_neurips}


% \title{Supplemental to {\it Differential Privacy Over Riemannian Manifolds}}
% \date{}

% \begin{document}
% \maketitle


\LARGE{Supplemental to {\it Differential Privacy Over Riemannian Manifolds}}
\nopagebreak
\normalsize
\section{Simulation details}
Simulations are done in Matlab on a desktop computer with an Intel Xeon processor at 3.60GHz with 31.9 GB of RAM running Windows 10.

\subsection{Computing the Fr\'echet mean}
We use a gradient descent algorithm to compute the Fr\'echet mean of a sample $D=\{x_1,x_2,\dots,x_n\}$. We initialize the mean $\hat{\mu}_0$ at any data point, take a small step in the average direction of the gradient of energy functional $F_2: \mcM \to \mathbb R$, and iterate. If $\hat \mu_{k-1}$ is the  mean in the $(k-1)$th iterate, in normal coordinates, the gradient is given by $v_k =\frac{1}{n}\sum_{i=1}^n \exp^{-1}_{\hat{\mu}_{k-1}}(x_i)$. Then, the  estimate of the Fr\'echet mean at iterate $k$ is $\hat{\mu}_k = \exp_{\hat{\mu}_{k-1}}(t_k v_k)$ where $t_k\in(0,1]$ is the step size. The algorithm is assumed to have converged once the change in the mean across subsequent steps is no longer significant, measured using the intrinsic distance $\rho$ on $\mcM$; that is, the algorithm terminates if $\rho(\mu_k,\mu_{k-1})<\lambda$ for some pre-specified $\lambda > 0$. We choose the step size $t_k=0.5$ and $\lambda = 10^{-5}$. In addition, one could set a maximum number of iterations for situations when the mean oscillates between local optima, and we set this at 500 but note that in our settings the algorithm typically converges in fewer than 200 iterations.

\subsection{SPDM simulations}
\subsubsection{Generating random samples within $B_r(m_0)$}\label{ss:SPDMGS}
Since $\mbPk$ can be identified with the set of $k \times k$ covariance matrices, we use the Wishart distribution $W(V,df)$ to generate samples from $\mbPk$, parameterized by a scale matrix $V$ and degrees of freedom $df>0$ such that if $X \sim W(V,df)$ then $EX=df\thinspace V$ . We set $V=\frac{1}{k} I_k$, where $I_k$ is the identity matrix and $df=k$. 

Recall that under the Rao-Fisher affine-invariant metric $\mbPk$ is negatively curved and thus the radius $r$ of ball $B_r(m_0)$ in Assumption 1 within which data $D$ is assumed to lie in is unconstrained. This results in samples from $W(\frac{1}{k} I_k,k)$ being centred at $I_k$, which can be viewed as a suitable value for $m_0$. It is possible, however, that certain samples from $W(\frac{1}{k} I_k,k)$ are at a distance (in terms of $\rho$) greater than $r$ from $m_0=I_k$ since the affine-invariant metric is not used in the definition of the Wishart, but this can always be adjusted by selecting a suitable radius $r$. A sample of size $n$ is thus generated by: (i) sampling $X \sim W(\frac{1}{k} I_k,k);$ (ii) retaining $X$ if $\rho(X,I_k)<r$ or (re-)sampling $X$ until distance is smaller than $r$. For our simulations, we set $r=1.5$ and $df=2$. 

%To generate a random sample in $\mbPk$ we use the Wishart distribution, since it randomly generates elements of $\mbPk$, in the following way. The Wishart distribution is parameterized by $V$ and $df$ with Euclidean distribution expected value of $df\cdot V$. For our simulations we set  $V=\frac{1}{k}I_k$, $df=k$, $k=2$, and $r=1.5$. We thus have distribution mean $I_k$ which we set as the center of the ball in the space of $\mbPk$. Although the elements of the sample must fall within the allotted radius, with our chosen parameters there is no guarantee that the Wishart will produce such an element. We thus check the distance on the manifold from $I_k$ to each element and redraw those which fall outside our radius.

\subsubsection{Radius in ambient space of symmetric matrices}
Let $Sym_k$ be the set of $k \times k$ symmetric matrices within which $\mbPk$ resides. In order to compare sensitivity of the proposed method using geometry of $\mbPk$ to one which considers only the ambient space $Sym_k$, the radius $r_E$ of a ball in $Sym_k$, with respect to the distance induced by the Frobenius norm $\|\cdot\|_2$, that in a certain sense `corresponds' to $r$ on $\mbPk$ needs to be ascertained. 

This amounts to determining how the distance $\rho(x,y)= \|\text{Log}(x^{-1/2} y x^{-1/2}) \|_{2}$ under the affine-invariant metric on $\mbPk$ compares to $\|x-y\|_2$ when $x,y \in \mbPk$. Since $m_0=I_k$, we can choose $y=I_k$ and compare $\|\text{Log}(x)\|_2$ with  $\| x - I_k\|_2$.
%Suppose we have generated a sample $D\subset\mbPk$ which lies on a ball with center $I_k$ and radius $r_m$. (We add the $m$ subscript to accentuate that this is the radius on the manifold.) The question we aim to answer in this section is, how does $r_m$ compare to the radius of the data in the ambient space? This is vital since we are comparing privacy using and ignoring the manifold structure, thus we must have comparable examples.

%Let $Sym_k$ denote the space of symmetric $k\times k$ matrices. First note that $\mbPk\subset Sym_k$. While we can consider the ambient space of $\mbPk$ to simply be $k\times k$ matrices, we use $Sym_k$ since under the Riemannian metric it is a tangent space and it preserves some structure to our data. So, let $x,y\in\mbPk$. Then the distance between $x$ and $y$ on the manifold is given by
%\[
%d(x,y) = 
%\|  \text{Log}(x^{-1/2} y x^{-1/2}) \|_{2}
%\]
%where $\| \cdot \|$ is the Frobenius norm for matrices. The question is how does this distance compare to the Euclidean norm $\|x - y \|^2$?


%Since we are taking the ball centered at the identity matrix, this means that we are interested in comparing
%\[
%\|\text{Log}(x)\|_2 \qquad \text{and} \qquad \| x - I\|_2. 
%\]
In particular, we seek to find the smallest Euclidean ball in $Sym_k$ that contains the geodesic ball $B_r(I_k)$ in $\mbPk$, and we accordingly define the radius of the Euclidean ball $r_E$ to be
\[
r_E = \sup_{x \in \mbPk:\| \text{Log}(x)\| \leq r} \|x - I\|.
\]
%the radius of the corresponding Euclidean ball centered at $I_k$ with radius $r_E$. 
Expressing $x$ in its diagonal basis following a suitable change of coordinates leaves $\|\text{Log}(x)\|$ and $\|x- I\|$ unchanged, and hence 
\[
r_E^2 = \sup_{\lambda: \sum_i \log(\lambda_i)^2 \leq r^2} \sum_i (\lambda_i - 1)^2,
\]
where $\lambda_i>0, i=1,\ldots,k$ are the eigenvalues of $x$. 

\begin{proposition}
$r_E = e^r -1$.
\end{proposition}
\begin{proof}
Let $u_i=\log \lambda_i, i=1,\ldots,k$. Consider the value of the objective function with the vector 
\[(u_1,u_2,u_3,\ldots,u_k)=\left(\sqrt{u_1^2+u_2^2},0,u_3,\ldots,u_k\right).\]
%$u_1 = \log(\lambda_1)$ and $u_2 = \log(\lambda_2)$, the first two eigen vectors, versus placing all of the weight in the first coordinate.  In other words, we compare $(u_1,u_2)$ against $(\sqrt{u_1^2 + u_2^2},0).$  The remaining $\lambda_3,\dots$ can take whatever value they like.  
The reason behind assuming such a structure for the vector of eigenvalues is that if we can show that the value of objective function increases by replacing $(u_1,u_2)$ by $(\sqrt{u_1^2 + u_2^2},0)$, then by symmetry the objective function will be maximized by placing all of the weight in the first coordinate and setting all remaining coordinates to $\lambda_i = 1$.  Consider a Taylor expansion of each of the terms (assume wlog that $u_i \geq 0$):
\begin{align}
    (e^{u_i} - 1)^2
    = \left(
    \sum_{n=1}^\infty \frac{u_i^n}{n!}
    \right)^2
    = \sum_{n, m} \frac{u_i^{n+m}}{n! m!}
\end{align}
versus
\begin{align}
    (e^{\sqrt{u_1^2+u_2^2}} - 1)^2
    = \left(
    \sum_{n=1}^\infty \frac{(u_1^2+u_2^2)^{n/2}}{n!}
    \right)^2
    = \sum_{n, m} \frac{(u_1^2+u_2^2)^{(n+m)/2}}{n! m!}.
\end{align}
We wish to establish that
\[
\sum_{n, m} \frac{(u_1^2+u_2^2)^{(n+m)/2}}{n! m!}
\geq 
\sum_{n, m} \frac{u_1^{n+m}+u_2^{n+m}}{n! m!}\thickspace.
\]
This will hold if 
\[
(u_1^2+u_2^2)^{(n+m)/2}
\geq u_1^{n+m}+u_2^{n+m},
\]
or equivalently
\[
u_1^2+u_2^2 \geq \left((u_1^2)^{(n+m)/2}+(u_2^2)^{(n+m)/2}\right)^{2/(n+m)}.
\]
However, since $n+m \geq 2$, this follows immediately from the triangle inequality for $\ell_p$ spaces.
\end{proof}


\subsection{Sphere simulations involving spheres}
\subsubsection{Generating samples within $B_r(m_0)$}
\label{ss:SphereGS}
We use polar coordinates to sample from a $d=2$-dimensional sphere $\mathcal S^2_1$ of radius one (thus $\kappa=1$). Let $(\theta,\phi)$ be the pair of polar and azimuthal angles, respectively, where $\theta\in[0,\pi]$ and $\phi\in[0,2\pi)$. We uniformly sample on $\theta\in[0,r]$ and $\phi\in[0,2\pi)$ with $r=\pi/8$. This results in data concentrated about the north pole ($m_0)$, with increasing concentration towards the north pole. %We note that uniform sampling on the polar coordinates does not generate uniform sample on $S^2_1$ and we make no such claim.
\subsubsection{Radius in ambient space }
Suppose we have a dataset $D$ on the unit sphere, $\mathcal S^d_1$, centered at $m_0$ with (manifold) radius $r$. As with SPDM, we need to determine a suitable ball of radius $r_E$ in Euclidean space that contains the geodesic ball of radius $r$ on $\mathcal S^d_1$. 
%We can embed the data into $\mbR^3$ but then we need to compute the radius of the corresponding Euclidean ball. For this manifold 
To determine $r_E$, we simply need to convert $r$, which corresponds to arc length, to the chord length (from $m_0$ to the boundary of the ball).
That is, since the sphere radius equals 1, $r_E=2 \sin(\frac{r}{2})$.% where $\alpha$ is the angle subtended at the origin of $\mathbb R^3$ by $m_0$ and a point on the boundary of $B_r(m_0)$. 
%We have that the angle $\alpha=\frac{r_M 2\pi}{2r_S\pi}=\frac{r_M}{r_S}$. 
With $r=\pi/8$ we obtain $r_E=2\sin(\pi/16)$. %since $\alpha=\frac{2\pi r}{2\pi}=r$.

\subsection{Sampling from the Euclidean Laplace} \label{ss:euc_lap}
We discuss how to sample from K-norm mechanism with the $\mathbb \ell_2$ norm $|\cdot|_2$ (i.e. the Euclidean Laplace) on $\mathbb R^d$.  First, wlog we can take $\bar x = 0$ and $\sigma =1$ as we can clearly generate from a standardized distribution and then translate/scale the result.  So the goal is to sample from 
\[
f(y) \propto e^{- |y|_2 }.
\]
Evidently, $f$ is a member of the elliptical family of distributions. We thus sample a vector $y=(y_1,\ldots,y_d)$ from $f$ by sampling a direction uniformly on the $(d-1)$-dimensional unit sphere $\mathcal S_1^{d-1}$ and then, independently, sampling a radius $r>0$ from an appropriate distribution. To determine this distribution, let 
 \begin{align*}
 & y_1 = r  \cos(\theta_1) \\
 & y_2 = r \sin(\theta_1) \cos(\theta_2), \\
 & \vdots \\
 & y_{d-1} = \sin(\theta_1) \sin(\theta_2) \dots \cos(\theta_{d-1}) \\
 & y_d = \sin(\theta_1) \dots \sin(\theta_{d-1}).
 \end{align*}
 Then the density $f$ assumes the form
\[
f(r,\theta_1,\dots, \theta_d)
= e^{-r} r^{d-1} \sin^{d-2}(\theta_1) \dots \sin(\theta_{d-1}).
\]
Since $f$ factors into a function of $r$ and a function of the angles, the distribution of $r$ is proportional to $r^{d-1} e^{-r}$, which is just the Gamma distribution $\Gamma(d,1)$ with parameters $\alpha = d$ and $\beta= 1$. Thus, to sample a value from $f$:
\begin{enumerate}
    \item sample a direction $U$ uniformly from $\mathcal S^{d-1}$;
    \item sample a radius $R$ from $\Gamma(d,1)$ distribution;
    \item set $Y = \bar x + R \sigma U$.
\end{enumerate}
Then $Y$ will be a draw from the $d$-dimensional Euclidean Laplace with scale $\sigma$ and center $\bar x$. In order to sample $U$ from $\mathcal S_1^{d-1}$, we use the well-known fact that if $X \sim N_d(\bm 0_d,I_d)$ then $U:=X/ |X|_2$ follows a uniform distribution on $S^{d-1}$.
\begin{comment}
\subsection{Sampling from the Laplace on the sphere $\mathcal S^{d}_1$}
First, notice that under our framework, the Riemannian volume measure on $\mathcal S^d_1$ just corresponds to the uniform measure.  
Thus, to sample from the Laplace on $\mathcal S^{d}_1$ we use a rejection sampler with a uniform proposal density. Let $X\sim f$, be a draw from the uniform distribution on $\mathcal S_1^{d}$. We aim to accept/reject draws from $f$ to produce samples $Y\sim g:= C^{-1}_{\eta,\sigma}\text{exp}(-\rho(\eta,x)/\sigma)$, where $\rho$ is the arc distance on the sphere.% $Y$ can be sampled as described above. 
%[\blue{I couldn't follow the exposition below concerning $M$}].
%We sample from the uniform on the sphere by sampling from three random normal distributions $Y_1,Y_2,Y_3\sim\text{N}(0,1)$, stacking these as a vector $y=[y_1,y_2,y_3]'$, and normalizing the vector $y\leftarrow y/\|y\|$ as discussed in \cite{muller1959note}. 
%
We follow a standard rejection sampling schematic.
%
\begin{enumerate}
\item Draw $X \sim f$, uniformly on $\mathcal S^d_1$.  For convenience, we took $X = Z/|Z|_2$, where $Z$ was a vector of standard normals.
\item Accept $X=x$ and set $Y=x$ with probability $\exp(- \rho(\eta,x)/\sigma)$.  Otherwise reject $x$ and return to step (1).
\item Repeat steps (1) and (2) until the desired sample size has been reached.
%Compute $\frac{f(y)}{Mg(y)}$ where $M=\sup_{y \in \mathcal S^d_1} \frac{f(y)}{g(y)}$. 
%Since, by construction, $f(y)$ is constant then $\frac{f(y)}{Mg(y)}=\text{exp}(-\rho(\eta,y)/\sigma)$. Thus, to sample from the Laplace on the sphere, we simply generate a point from the uniform on the $S_1^2$, then evaluate $\text{exp}(-\rho(\eta,y)/\sigma)$ and if this quantity is larger than we accept it as a random sample from the Laplace.
\end{enumerate}
To see why $\exp(-\rho(\eta,x)/\sigma)$ is a suitable acceptance probability, recall that in rejection sampling we require an $M \in \mathbb R$ such that
\[
\sup_{x} \frac{g(x)}{M f(x)} \leq 1,
\]
in which case one can set the acceptance probability to $g(x)/M f(x)$.  In this case, $f(x) \equiv c^{-1}$ is constant since it is uniform and thus we can take $M = C_{\eta,\sigma}^{-1} c$, which yields
\[
\frac{g(x)}{M f(x)}
= \exp(-\rho(\eta,x)/\sigma) \leq 1,
\]
as required.
\end{comment}
%--------------------------------------------------------------
\subsection{Sampling from the Laplace on the sphere $\mathcal S^{d}_1$}
To sample from the Laplace on $\mathcal S^{d}_1$ we generate a Markov chain by using a Metropolis-Hastings random walk. At each step $n$ we generate a proposal $x'$ by first randomly drawing a vector $v$ in the current tangent space, $T_{x_n}\mathcal{S}_1^d$, then move on the sphere using the exponential map and said vector, $f(x'|x_n)=\exp_{x_n}v$. 
%[\red{is this the transition density or the update step?}]
To draw $v$ we uniformly sample on a ball centered at the current step $x_n$ with radius $\sigma$ by drawing a vector from $N_3(0_3,I_3)$, scaling the resulting vector to have length $\sigma$, and projecting the vector onto the tangent space of $x_n$. This projection ensures that $\|v\|\leq\sigma$, which we take to be much smaller than the injectivity radius. Further, $v$ is not uniform in $T_{x_n}\mathcal S^{d}_1$, but since we use a Metropolis-Hastings algorithm, we only require symmetry is satisfied. One can sample vectors on the required tangent space in several manners, the proposed method is chosen for computational ease. 

We aim to accept/reject draws from $f$ to produce a Markov chain with stationary density $C^{-1}_{\eta,\sigma}\text{exp}(-\rho(\eta,x)/\sigma)$, where $\rho$ is the arc distance on the sphere. We follow a standard Metropolis-Hastings schematic.

\begin{enumerate}
\item Initialize $x_0=\eta$.
\item In the $n$th iteration, draw a vector in $T_{x_n}\mathcal S^{d}_1$, the tangent space of $x_n$, as described earlier denoted as $v$.
\item Generate a candidate $x'$ by letting $x'=\exp_{x_n}v$. 
\item Accept $x'$ and set $x_{n+1}=x'$ with probability $\exp(- \rho(\eta,x')/\sigma)/\exp(- \rho(\eta,x_n)/\sigma)$. Otherwise, reject $x'$ and generate another candidate by returning to previous step.
\item Return to step 2 until one has generated a sufficiently long chain.
\end{enumerate}
 The final sample is chosen based on a burn-in period of 10 000 steps and jump width of 100 to avoid correlated adjacent steps in the chain.

 \section{Bounding Distances on the Tangent Space}
 To complete Theorem 2 we need a bound on the distance
 \[
 \|\exp_{m}^{-1}(x) - \exp_{m}^{-1}(y)\|_m,
 \]
 which holds uniformly across all $m,x,y \in B_r(m_0)$; in particular, we seek a Lipschitz bound that holds uniformly over $B_r(m_0)$. 

\begin{lemma}
Under the assumptions of Theorem 2, for $x,y,m \in B_r(m_0)$ we have
\[
\|\exp_{m}^{-1}(x) - \exp_{m}^{-1}(y)\|_m
\leq 2r (2 - h(r, \kappa)).
\]
\end{lemma}
\begin{proof}
We first establish that the inverse exponential map at a fixed $m \in B_r(m_0)$ is Lipschitz. The map $\exp_m:T_xM \to \mcM$ when restricted to a ball $B$ of radius $r$ around the origin is a diffeomorphism since $\text{inj} \ m < r$. The inverse $\exp_m^{-1}$ is differentiable on $\exp_m(B)$. Let $N_m=\exp_m(B) \cap  B_r(m_0)$ and consider a minimizing geodesic $\gamma:[0,1] \to \mcM$ starting at $m$ that lies entirely in $N_m$.

The derivative $\text{D} \exp_m^{-1}$ is the value of $\dot J(1)=\frac{\text{D}}{ds}\frac{d}{dt}c_m(s,t)\Big|_{s=1}$, where $J(s)=\frac{d}{dt} c_m(s,t)$ is the Jacobi field  along $s \mapsto c_m(s,t)=\exp_m\{s \exp_m^{-1}(\gamma(t))\}$, with $J(0)=0$ and $J(1)=\dot \gamma(t)$. When restricted to the (compact) closure of $B$,  the map $v \mapsto \|\text{D}\exp_m^{-1} v \|_m$ is bounded above by $C(m)<\infty$. 

Let $\Gamma:=\exp_m^{-1}(\gamma)$. Comparing lengths of $\gamma$ and $\Gamma$ we obtain
\[
L(\Gamma)\leq C(m) \int_0^1 \|\gamma'(t)\|_{\gamma(t)}\text{d}t=C(m) L(\gamma),
\]
since $\|\cdot\|_m$ is continuous. Since distances are obtained by minimising lengths of paths of curves, $\exp_m^{-1}$ is Lipshcitz with constant $C(m)$ on $N_m$. However, under the assumptions of Theorem 2, from Jacobi field estimates A5.4, when used in conjunction with Corollary 1.6, in \footnote{H. Karcher. \emph{Riemannian center of mass and mollifier smoothing}, Communications in Pure and Applied Mathematics (1977), 509-541.}, we get
%To find $C$, note that for a fixed $m$, $\nabla \frac{1}{2} d^2(m,y)=-\exp_m^{-1}(y)$ and  the derivative of the inverse exponential can thus be interpreted in two ways:
%\begin{enumerate}
 %   \item An operator $T_m M \to T_m M$ defined as $v \mapsto \nabla _v \nabla \frac{1}{2} d^2(m,y)$.
 %   \item As $\dot J(1)=\frac{\text{D}}{ds}\frac{d}{dt}c_m(s,t)\Big|_{s=1}$, where $J(s)=\frac{d}{dt} c_m(s,t)$ is the Jacobi field  along $s \mapsto c_m(s,t)=\exp_m\{s \exp_m^{-1}(\gamma(t))\}$ for a geodesic $\gamma:[0,1] \to B_{m_0}(r)$ with $J(0)=0$ and $J(1)=\dot \gamma(t)$. 
%\end{enumerate}
%Combing through two papers \footnote{H. Karcher. \emph{Riemannian center of mass and mollifier smoothing}, Communications in Pure and Applied Mathematics (1977), 509-541.}\footnote{H. Le. \emph{Locating Frechet means with applications to shape spaces}, Advances in Applied Probability (2001), 33,324-338.} that use both interpretations, we get%, skipping details, 
%the following bound on the operator norm on $\text{D}\exp_x^{-1}$ as
\[
C(m) \leq \sup_{v \in T_m M, \|v\|_m=1}\|\text{D}\exp_m^{-1}v \|_{m}\leq 
\left\{
\begin{array}{cc}
2-h(r,\kappa)     &  \text{if } \kappa>0 \\
1     & \text{if } \kappa \leq 0,
\end{array}
\right.
\]
where $h(r,\kappa)$ is as defined in Theorem 2. As a consequence,
\[
\|\exp_m^{-1}(x)-\exp_m^{-1}(y)\|_m \leq [2-h(r,\kappa)]d(x,y) \leq 2r[2-h(r,\kappa)],
\]
as desired.
%In particular, for the unit sphere with $\kappa=1$, $1<[2-h(r,1)]\leq 2$ for $0<r \leq \pi/4$. The upper bound seems to work as needed, but I need to check my calculations again. 
\end{proof}


\subsection{An Empirical Bound on the Sensitivity for $\mathcal S^{d}_1$}
The sensitivity is bound as  $ \rho(\bar x, \bar x') \leq \frac{2r(2-h(r,\kappa))}{n h(r,\kappa)}$ where $h(r,\kappa)$ is a function of the radius of the ball $B_r(m_0)$ and $\kappa$ the sectional curvature of the manifold. The correction factor in the numerator, which is only present for positively curved manifolds, is not very tight for large radius ball. From the theorem we see that this correction factor comes from $\|\exp^{-1}_{m}(x)-\exp^{-1}_{m}(y)\|\leq 2r[2-h(r,\kappa)]$, so we consider this norm in the case of the unit sphere. 

Given a ball $B_r(m_0)$ and any three points $x_1,x_2,x_3\in B_r(m_0)$, we wish to find an empirical bound on $\|\exp^{-1}_{x_1}(x_2)-\exp^{-1}_{x_1}(x_3)\|$. To do this we create a uniformly spaced grid on the boundary of $B_r(m_0)$ to produce a set $\{x_i\}$. We then fix an arbitrary point, say $x_1$, and compute $\max_{i,j}  \|\exp^{-1}_{x_1}(x_i)-\exp^{-1}_{x_1}(x_j)\|$. Because of the symmetry of the ball on the sphere, one can fix the footpoint and search over all other points.
\begin{figure}
    \centering
    \includegraphics[height=2.5in]{radiusVsBound}
    \caption{The x-axis represents the radius of $B_r(m_0)$. The blue line is $2r$, the red line is $2r(2-h(r,\kappa))$, and  the yellow line is $\max_{i,j} \|\exp^{-1}_{ x}(x_i)-\exp^{-1}_{x}(x_j)\|$.}
    \label{fig:Sensitivity}
\end{figure}
In Figure \ref{fig:Sensitivity} we display the radius of $B_r(m_0)$ as the x-axis, $2r$ in blue, $2r[2-h(r,\kappa)]$ in red, and $\max_{i,j} \|\exp^{-1}_{ x}(x_i)-\exp^{-1}_{x}(x_j)\|$ in yellow. We see that $2r<\max_{i,j} \|\exp^{-1}_{ x_1}(x_i)-\exp^{-1}_{x_1}(x_j)\|<2r(2-h(r,\kappa))$ however the inflation due to the the curvature is not as large as our bound. Rather than use the theoretical bound in the simulations of the sphere, we use the empirical bound.

 
 
 




% \end{document}








==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
